Ozone: Fully Out-of-Order Choreographies

Choreographic programming is a paradigm for writing distributed applications. It allows programmers to write a single program, called a choreography, that can be compiled to generate correct implementations of each process in the application. Although choreographies provide good static guarantees, they can exhibit high latency when messages or processes are delayed. This is because processes in a choreography typically execute in a fixed, deterministic order, and cannot adapt to the order that messages arrive at runtime. In non-choreographic code, programmers can address this problem by allowing processes to execute out of order -- for instance by using futures or reactive programming. However, in choreographic code, out-of-order process execution can lead to serious and subtle bugs, called communication integrity violations (CIVs). In this paper, we develop a model of choreographic programming for out-of-order processes that guarantees absence of CIVs and deadlocks. As an application of our approach, we also introduce an API for safe non-blocking communication via futures in the choreographic programming language Choral. The API allows processes to execute out of order, participate in multiple choreographies concurrently, and to handle unordered data messages. We provide an illustrative evaluation of our API, showing that out-of-order execution can reduce latency and increase throughput by overlapping communication with computation.

==> choral_macros.tex <==
\usepackage{listings}

\expandafter\patchcmd\csname \string\lstinline\endcsname{%
  \leavevmode
  \bgroup
}{%
  \leavevmode
  \ifmmode\mbox\fi
  \bgroup
}{}{%
  \typeout{Patching of \string\lstinline\space failed!}%
}


\lstdefinelanguage{Choral}{
  morekeywords={class,else,extends,if,implements,interface,new,null,private,%
      protected,public,abstract,final,static,return,super,this,try,catch,void, %
      enum,switch,case,default,throw,throws,with,forall,in},%
  otherkeywords={>>,::,@},
  sensitive,%
  escapechar=¦,
	morecomment=[l]//,%
	morecomment=[s]{/*}{*/},%
	morestring=[b]",%
  morestring=[b]',%
  moredelim=[is][]{\#}{\#}%
}[keywords,comments,strings]%

\lstdefinelanguage{comperr}{
  morekeywords={class,else,extends,if,implements,interface,new,null,private,%
      protected,public,abstract,final,static,return,super,this,try,catch,void, %
      enum,switch,case,default,throw,throws},%
  otherkeywords={>>,@},
  sensitive,%
	morecomment=[l]//,%
	morecomment=[s]{/*}{*/},%
	morestring=[b]",%
  morestring=[b]',%
  moredelim=[is][]{\#}{\#},
  moredelim=[is][\bfseries\color{sred}]{~}{~},
  moredelim=[is][basicstyle]{/~}{~/}
}[keywords,comments,strings]%


\usepackage[scaled=.85]{FiraMono}

\definecolor{sbase03}{HTML}{002B36}
\definecolor{sbase02}{HTML}{073642}
\definecolor{sbase01}{HTML}{586E75}
\definecolor{sbase00}{HTML}{657B83}
\definecolor{sbase0}{HTML}{839496}
\definecolor{sbase1}{HTML}{93A1A1}
\definecolor{sbase2}{HTML}{EEE8D5}
\definecolor{sbase3}{HTML}{FDF6E3}
\definecolor{syellow}{HTML}{B58900}
\definecolor{sorange}{HTML}{CB4B16}
\definecolor{sred}{HTML}{DC322F}
\definecolor{smagenta}{HTML}{D33682}
\definecolor{sviolet}{HTML}{6C71C4}
\definecolor{sblue}{HTML}{268BD2}
\definecolor{scyan}{HTML}{2AA198}
\definecolor{sgreen}{HTML}{859900}

\lstdefinestyle{solarized-light}{
  frame=none,
  breaklines=true,
  showstringspaces=false,
  tabsize=1,
  columns=fixed,
  mathescape=true,
  extendedchars=true,
  backgroundcolor=\color{sbase3},
  keywordstyle=\bfseries\color{sbase01},
  keywordstyle=[2]\bfseries\color{sbase01},
  stringstyle=\color{sviolet},
  numberstyle=\color{sviolet},
  identifierstyle=\color{sbase03},
  commentstyle=\color{sgreen},
  basicstyle=\color{sbase03}\ttfamily\lst@ifdisplaystyle\footnotesize\fi,
  moredelim=[is][\color{sblue}]{\#}{\#},
}


\usepackage[most]{tcolorbox}
\tcbuselibrary{listings}

\NewDocumentCommand{\newlang}{o m m m}{%
  \IfNoValueTF{#1}{\def\n{#2}}{\def\n{#1}}
  \expandafter\NewDocumentCommand\csname \n listing\endcsname{s O{} O{}}{%
	  \def\WithoutTitle{\tcblisting{
	          enhanced, %
	          %
	          before skip=\abovedisplayskip,
	          after  skip=\belowdisplayskip,
	          sharp corners=all,
	          boxrule=2pt,
	          boxsep=-.7em,
	          colframe=#4,
	          colback=sbase3,
	          title={},
	          listing only,
	          listing options={language=#2,numbers=left,style=solarized-light,##3},
	          ##2
 	  	}}%
  	\def\withTitle{\tcblisting{
         enhanced, %
         before skip=\abovedisplayskip,
         after  skip=\belowdisplayskip,
         sharp corners=all,
         boxrule=2pt,
         boxsep=-.7em,
         colframe=#4,
         colback=sbase3,
         detach title,
         finish={\node[anchor=south east, font=\footnotesize\itshape,
         text=sbase3,fill=#4] at (frame.south east) {#3 Code};},
         title={},
         listing only,
         listing options={language=#2,numbers=left,style=solarized-light,##3},
         ##2
   }}%
   \IfBooleanTF{##1}{\WithoutTitle}{\withTitle}}
  \expandafter\def\csname end\n listing\endcsname{\endtcblisting\noindent}
  \expandafter\def\csname\n\endcsname{\lstinline[language=#2,style=solarized-light]}
}

\newlang[chor]{choral}{Choral}{sblue}
\newlang[comm]{java}{Generated}{syellow}
\newlang[local]{java}{Local}{sbase01}
\newlang[blah]{java}{Java}{sbase1}
\newcommand{\annotation}[1]{{\color{sgreen!60!black}\texttt{#1}}}
\newcommand{\codeComment}[1]{{\color{sgreen}\texttt{#1}}}

\newcommand\code{\lstinline[language=Choral,style=solarized-light]}
\newcommand{\mcode}[1]{\hbox{\code{#1}}}


\newcommand{\Div}{\hspace{1.2ex}{\color{gray!80}\vline height 1em depth .3em width 1px}\hspace{1.2ex}}
\newcommand{\s}{{\color{lightgray}\cdot}}
\newcommand{\many}[1]{\overline{#1}}

\defann{hlNew}{\cb{green!30}\uline}
\defann{hlOpt}{\cb{gray!10}\dashuline}
\newcommand{\opt}[1]{\hlOpt*{\vphantom{\overline{\langle}}#1}} %
\newcommand{\diff}[1]{\hlNew*{\vphantom{\overline{\langle}}#1}}
\newcommand{\genW}{\mcode{\#A\#}}
\newcommand{\genWs}{\many{\genW}}
\newcommand{\at}{\mcode{@}}
\newcommand{\params}[1]{\langle#1\rangle}
\newcommand{\grammarTerm}[1]{\mathit{#1}}

\newcommand{\id}{\grammarTerm{id}}
\newcommand{\cst}{\grammarTerm{lit}}
\newcommand{\program}{\grammarTerm{P}}
\newcommand{\cu}{\grammarTerm{cu}}
\newcommand{\interface}{\grammarTerm{Interface}}
\newcommand{\class}{\grammarTerm{Class}}
\newcommand{\enum}{\grammarTerm{Enum}}
\newcommand{\Term}{\grammarTerm{Term}}

\newcommand{\ANN}{\grammarTerm{AN}}
\newcommand{\MOD}{\grammarTerm{MD}}

\newcommand{\FTP}{\grammarTerm{FTP}}
\newcommand{\TE}{\grammarTerm{TE}}
\newcommand{\FA}{\grammarTerm{FAcc}}

\newcommand{\MethodDef}{\grammarTerm{MDef}}
\newcommand{\VarDecl}{\TE\s \id}
\newcommand{\ClassConst}{\grammarTerm{CConst}}
\newcommand{\ClassField}{\grammarTerm{CField}}
\newcommand{\Stm}{\grammarTerm{Stm}}
\newcommand{\Exp}{\grammarTerm{Exp}}
\newcommand{\MethodInv}{\grammarTerm{MInv}}
\newcommand{\ExpChain}{\grammarTerm{EChain}}
\newcommand{\AsgOp}{\grammarTerm{AsgOp}}
\newcommand{\BinOp}{\grammarTerm{BinOp}}
\newcommand{\SwArg}{\grammarTerm{SwArg}}

\newcommand{\NewClass}{\grammarTerm{NewClass}}
\newcommand{\NewCase}{\grammarTerm{NewCase}}

\newcommand{\static}{\mcode{static}}
\newcommand{\new}{\mcode{new}}
\newcommand{\case}{\mcode{case}}
\newcommand{\switch}{\mcode{switch}}


\definecolor{auxFnColor}{rgb}{0.56, 0.0, 1.0}
\newcommand{\auxFn}[1]{{ \color{auxFnColor}\textsc{#1} }}
\newcommand{\worlds}[1]{\auxFn{worlds}(#1)}
\newcommand{\genWorlds}[1]{\worlds{#1}^{\Gamma}}
\newcommand{\idx}[1]{\auxFn{idx}(#1)}
\newcommand{\blank}{[blank]}

\def\solOpen{{\color{sblue}\llparenthesis}}
\def\solClose{{\color{sblue}\rrparenthesis}}
\newcommand{\sol}[1]{\solOpen #1 \solClose}
\newcommand{\genSol}[1]{\sol{#1}^{\mcode{\#A\#},\Gamma}}
\newcommand{\genSolP}[1]{\sol{#1}^{\mcode{\#A'\#},\Gamma}}

\newcommand{\unit}{\mcode{Unit}}
\newcommand{\uid}{{{\color{auxFnColor}\texttt{.id}}}}
\newcommand{\unitq}[1]{\auxFn{unit}(#1)}
\newcommand{\genUnitq}[1]{\unitq{#1}^{\genW,\Gamma}}

\newcommand{\mergeSign}{{\color{red}{\sqcup}}}
\newcommand{\bigMergeSign}{{\color{red}{\dot\bigsqcup}}}
\newcommand{\solMerge}{\mathbin{\mergeSign}}

\newcommand{\llambda}[1]{\lambda\left(#1\right)}
\newcommand{\scoped}[2]{#1\downharpoonright#2}

\newcommand{\headAndTail}[1]{\auxFn{ht}(#1)}

\newcommand{\unitSol}[1]{{\color{red}\text{[\![}} #1 {\color{red}\text{]\!]}}}
\newcommand{\unitSolChange}[1]{\unitSol{#1}^{\color{red}\star}}
\renewcommand{\paragraph}[1]{\noindent\textit{#1.}\ \ignorespaces}
\newcommand{\megapar}[1]{\noindent\textbf{#1.}\ \ignorespaces}


==> preamble.tex <==
\usepackage{xparse}
\usepackage{etoolbox}
\usepackage{environ}

\makeatletter
\newcommand{\IfLabelExistsTF}[3]{\@ifundefined{r@#1}{#3}{#2}}
\newcommand{\IfLabelExistsT}[2]{\IfLabelExistsTF{#1}{#2}{}}
\newcommand{\IfLabelExistsF}[2]{\IfLabelExistsTF{#1}{}{#2}}
\newcommand{\IfDefTF}[3]{\@ifundefined{#1}{#3}{#2}}
\newcommand{\IfDefT}[2]{\IfDefTF{#1}{#2}{}}
\newcommand{\IfDefF}[2]{\IfDefTF{#1}{}{#2}}
\makeatother




\newcommand\scalemath[2]{\scalebox{#1}{\mbox{\ensuremath{\displaystyle #2}}}}

\usepackage{subfiles}
\usepackage{xr}
\usepackage{currfile}

\ifdefined\docroot\else
 \let\docroot\currfilepath
\fi

\newcommand\IfDocRootTF[2]{%
 \ifcurrfilepath{\docroot}{#1}{#2}%
}
\newcommand\IfDocRootT[1]{\IfDocRootTF{#1}{}}
\newcommand\IfDocRootF[1]{\IfDocRootTF{}{#1}}


%\usepackage[x11names,rgb,html]{xcolor}

\colorlet{textcolor}{.}
\newcommand\usecolor[2]{\begingroup%
  \colorlet{uc@saved}{.}
  \color{#1}#2\color{uc@saved}
\endgroup}
\newcommand\cboxed[2]{\begingroup%
  \colorlet{cb@saved}{.}%
  \color{#1}%
  \boxed{\color{cb@saved}#2}%
\endgroup}

\usepackage{tikz}
\usetikzlibrary{calc}
\usetikzlibrary{positioning}
\usetikzlibrary{tikzmark}
\usepackage{graphicx}
\usepackage{pgfplots}

%\usepackage[british]{babel}


\usepackage{amsmath}
\usepackage{amsthm}
\usepackage{amsfonts}
\usepackage{centernot}
\usepackage{scalerel}
\usepackage{stmaryrd}
\SetSymbolFont{stmry}{bold}{U}{stmry}{m}{n}
\usepackage{mathtools}


\makeatletter
\DeclareFontEncoding{LS2}{}{\@noaccents}
\makeatother
\DeclareFontSubstitution{LS2}{stix}{m}{n}

\DeclareSymbolFont{largesymbolsstix}{LS2}{stixex}{m}{n}

\DeclareMathDelimiter{\lbrbrak}{\mathopen}{largesymbolsstix}{"EE}{largesymbolsstix}{"14}
\DeclareMathDelimiter{\rbrbrak}{\mathclose}{largesymbolsstix}{"EF}{largesymbolsstix}{"15}

\allowdisplaybreaks

\usepackage{array}
\usepackage{xtab}
\usepackage{booktabs}
\usepackage{multicol}

\usepackage{float}
\usepackage{placeins}
\usepackage{wrapfig}

\usepackage[inline]{enumitem}

\usepackage{hyperref}
\usepackage{nameref}

%\usepackage[capitalise,nameinlink,noabbrev]{cleveref}
\makeatletter
\newcommand{\customlabel}[4][0]{%
  \protected@write\@auxout{}{\string\newlabel{#3}{{#4}{\thepage}{#4}{#3}{}}}%
  \protected@write\@auxout{}{\string\newlabel{#3@cref}{{[#2][#1][#1]#4}{\thepage}}}%
}
\newcommand{\phantomlabel}[4][0]{%
  \customlabel[#1]{#2}{#3}{#4}%
  \hypertarget{#3}{}%
}
\newcommand{\crefv}[1]{%
  \begingroup\@cref@compressfalse\@cref@sortfalse\cref{#1}\endgroup%
}
\newcommand{\Crefv}[1]{%
  \begingroup\@cref@compressfalse\@cref@sortfalse\Cref{#1}\endgroup%
}
\newcommand{\crefabbrev}[1]{%
  \begingroup\@cref@abbrevtrue\cref{#1}\endgroup%
}
\makeatother

\AtEndPreamble{\hypersetup{
  final,
}}


\usepackage[
  disable,     %
  obeyFinal,   %
  textwidth=\marginparwidth,
  textsize=footnotesize,
  colorinlistoftodos,
  prependcaption
]{todonotes}
\newcommand{\unsure}[2][]{\todo[linecolor=red,backgroundcolor=red!25,bordercolor=red,#1]{#2}}
\newcommand{\change}[2][]{\todo[linecolor=blue,backgroundcolor=blue!25,bordercolor=blue,#1]{#2}}
\newcommand{\info}[2][]{\todo[linecolor=cyan,backgroundcolor=cyan!25,bordercolor=cyan,#1]{#2}}
\newcommand{\improvement}[2][]{\todo[linecolor=green,backgroundcolor=green!25,bordercolor=green,#1]{#2}}

\makeatletter
\if@todonotes@disabled
\else %
\paperwidth=\dimexpr \paperwidth + 6cm\relax
\oddsidemargin=\dimexpr\oddsidemargin + 3cm\relax
\evensidemargin=\dimexpr\evensidemargin + 3cm\relax
\marginparwidth=\dimexpr \marginparwidth + 3cm\relax
\AtBeginDocument{\todo{Disable todos before submission}}
\fi
\makeatother


\makeatletter
\def\new@acronym#1#2{\expandafter\def\csname#1\endcsname{{\upshape #2}\xspace}}
\def\new@acronymexp#1#2{\expandafter\def\csname#1@exp\endcsname{{#2}}}
\NewDocumentCommand{\newacronym}{o m o}{%
  \IfNoValueTF{#1}{\def\n{#2}}{\def\n{#1}}
  \new@acronym{\n}{#2}
  \IfNoValueF{#3}{\new@acronymexp{\n}{#3}}
}
\def\expandacronym#1{\csname#1@exp\endcsname}
\makeatother

\DeclareMathOperator{\dom}{dom}
\DeclareMathOperator{\cod}{cod}
\DeclareMathOperator{\img}{img}


\def\crel#1{\mathrel{\mathcal{#1}}}

\def\disjoint{\mathrel{\#}}

\let\defeq\triangleq
\edef\defiff{\stackrel{\triangle}{\iff}}

\makeatletter
\newcount\c@repeat@count
\newcommand{\crepeat}[2]{%
  \begingroup
  \c@repeat@count=\z@
  \@whilenum\c@repeat@count<#1\do{#2\advance\c@repeat@count\@ne}%
  \endgroup
}
\makeatother

\newenvironment{bnftable}[3][]
	{\par\vspace{\abovedisplayskip}\indent%
	  \sbox0{$#2 \Coloneqq {}$}%
	  \sbox1{$#3$}%
	  \begin{xtabular}{%
	      >{\raggedleft$}m{\wd0}<{$}%
	      >{\raggedright$#1\begingroup}m{\wd1}<{\endgroup$}%
	      >{\quad\it}l<{}}}
	{\end{xtabular}\vspace{\belowdisplayskip}\par\noindent}

\usepackage[normalem]{ulem}
\makeatletter
\def\cb#1#2#3{{\fboxsep=0pt\colorbox{#1}{\vphantom{\uline{#3}}#2{#3}}}}
\def\defann#1#2{%
	\expandafter\def\csname#1\endcsname{%
		\def\ann@####1{\hbox{#2{\ensuremath{####1}}}}%
		\def\ann@@####1{#2{####1}}%
		\@ifstar{\ann@}{\ann@@}%
	}}
\makeatother

\newcommand{\newtext}{\color{blue}}
\newcommand{\oldtext}{\color{black}}
\newcommand{\pleaseCheck}{\todo{Remove this comment when the new text has been checked.}}
\let\newtext\relax
\let\oldtext\relax


